CrossNet: Latent Cross-Consistency for Unpaired Image Translation

Recent GAN-based architectures have been able to deliver impressive performance on the general task of image-to-image translation. In particular, it was shown that a wide variety of image translation operators may be learned from two image sets, containing images from two different domains, without establishing an explicit pairing between the images. This was made possible by introducing clever regularizers to overcome the under-constrained nature of the unpaired translation problem. In this work, we introduce a novel architecture for unpaired image translation, and explore several new regularizers enabled by it. Specifically, our architecture comprises a pair of GANs, as well as a pair of translators between their respective latent spaces. These cross-translators enable us to impose several regularizing constraints on the learnt image translation operator, collectively referred to as latent cross-consistency. Our results show that our proposed architecture and latent cross-consistency constraints are able to outperform the existing state-of-the-art on a variety of image translation tasks.

==> Bokeh.tex <==
\subsection{Depthless Bokeh}
With the recent explosion in mobile phones that are equipped with dual sensors (or more), many intriguing features which involve depth information have been released publicly. The small aperture of mobile phones makes the depth of field large, yielding images where almost everything is in focus. Dual sensor phones are able to extract an auxiliary depth map, enabling features such as synthetic shallow depth of field.
%The very useful depth map may be leveraged for creating a synthetic shallow depth of field by gradually blurring objects according to their distance from an object one wishes to leave focused.

However, dual sensors come at a cost, providing good motivation for alternative approaches for synthetic shallow depth-of-field.
%employing this dual sensor approach for achieving the synthetic shallow depth of field is costly since it increases the Bill of Materials for the phone manufacturer. Thus, algorithms attempting to create a synthetic shallow depth of field given an Extended depth of Field (an almost fully in focus input) have been pursued. 
For example, Wadhwa et al.~\shortcite{wadhwa2018synthetic} propose an algorithm for achieving synthetic shallow depth-of-field with a single-camera mobile phone, through training a neural network on a foreground-background segmentation task. This in turn requires carefully annotated masks, a costly process.

Using our approach, we are able to translate images acquired with a large f-number lens into ones that appear to have a shallow depth-of-field. We collect two sets of images, ones which were captured using a large f-number lens and ones captured with a small f-number. \dl{where did we get them from? How many?} Following the exact same procedure as described in the previous sections \dl{where did we describe the procedure?}, we train \OurName on these two sets, and in a completely unsupervised manner \dl{can't say that... fully automatic after training is not the same as unsupervised...}, yield shallow depth-of-field outputs. In order to limit domains $A$ and $B$, so that small sets are representative of their distribution, we apply our Bokeh \dl{mention Bokeh now for the first time! no explanation/definition of the term} on selfies. This is similar to the current very popular "portrait mode" present in iPhone and Samsung Galaxy series, also enforcing that the enhanced image is a selfie. Thus, our manually collected image sets are selfies taken with either a large or a small F-Number lens. 
\dl{Please rewrite the entire above paragraph, while shortening it...}

In Figure \ref{tab:SDOFZoom} we present our results, compared with CycleGAN \shortcite{zhu2017unpaired} and MUNIT \shortcite{huang2018multimodal}. We zoom into crops of the results and put an emphasis on the differences between \OurName and the two competing methods. Firstly, it is shown that CycleGAN tends to suffer from checkerboard artifacts. It is also quite noticeable that CycleGAN isn't able to properly separate between the foreground and background and either blurs improperly or doesn't blur the desired regions. Another interesting artifact is CycleGAN's inability to preserve the proper colors in the blurry output, showing a tendency of creating a greenish hue. Applying MUNIT requires a style image from the target domain as input. In the results shown hereby, we fed the style input by randomly selecting a style image from our target image set, as proposed by the paper's provided implementation. The results show that although MUNIT is a very powerful approach for creating a rich variety of images from the target domain, it is less suitable for this task, since it undesirably translates the palette and textures, which is not required for this application.

We note that our approach is also not artifact-free. The boundaries between blurry and sharp regions are not always perfect and over-sharpening of the foreground is visible. Our intuition is that this is caused by the limited size of the dataset which we collected, consisting of ~500 images from each domain. Moreover, the realization that selfie poses are very diverse increases the need for a larger dataset for properly representing the domain's distribution.
We provide more results in the supplementary material.

\begin{figure}[ht]
\begin{tabular}[t]{cccc}

Input & \OurName & CycleGAN & MUNIT \\

\includegraphics[width=0.2\linewidth]{Figures/SDOF_0020_real_B.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0020_fake_A_Ours.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0020_fake_A_CG.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0020_fake_A_MUNIT.png} \\

\includegraphics[width=0.2\linewidth]{Figures/SDOF_0020_real_B_Xs44_Xe143_Ys75_Ye177.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0020_fake_A_Ours_Xs44_Xe143_Ys75_Ye177.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0020_fake_A_CG_Xs44_Xe143_Ys75_Ye177.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0020_fake_A_MUNIT_Xs44_Xe143_Ys75_Ye177.png} \\

\includegraphics[width=0.2\linewidth]{Figures/SDOF_0086_real_B.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0086_fake_A_Ours.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0086_fake_A_CG.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0086_fake_A_MUNIT.png} \\

\includegraphics[width=0.2\linewidth]{Figures/SDOF_0086_real_B_Xs1_Xe95_Ys133_Ye217.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0086_fake_A_Ours_Xs1_Xe95_Ys133_Ye217.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0086_fake_A_CG_Xs1_Xe95_Ys133_Ye217.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0086_fake_A_MUNIT_Xs1_Xe95_Ys133_Ye217.png} \\

\includegraphics[width=0.2\linewidth]{Figures/SDOF_0458_real_B.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0458_fake_A_Ours.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0458_fake_A_CG.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0458_fake_A_MUNIT.png} \\

\includegraphics[width=0.2\linewidth]{Figures/SDOF_0458_real_B_Xs66_Xe162_Ys2_Ye89.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0458_fake_A_Ours_Xs66_Xe162_Ys2_Ye89.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0458_fake_A_CG_Xs66_Xe162_Ys2_Ye89.png} &
\includegraphics[width=0.2\linewidth]{Figures/SDOF_0458_fake_A_MUNIT_Xs66_Xe162_Ys2_Ye89.png}

\end{tabular}
\caption{Results of our Depthless unsupervised Bokeh. We depict the input (left most), our result (second column from the left) and the competing methods CycleGAN and MUNIT (two right columns correspondingly). Every odd row shows the full image while the even rows show a zoom into regions in the full images. Note the checker artifacts which CycleGAN undesirably created in the first two rows of results, and the improper green hue which is noticeable in the 4 bottom most rows. Although they have shown very impressive translation results, MUNIT doesn't seem like an image-to-image translation method suitable for enhancement purposes, since it undesirably translates the palette and textures.}
\label{tab:SDOFZoom}
\end{figure}


\begin{figure*}[ht]
\begin{tabular}{cccccc}


Input & Ours & CG & Input & Ours & CG\\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0007_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0007_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0007_fake_A_CG.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0013_real_B.png} & %\includegraphics[width=0.1\linewidth]{Figures/SDOF_0013_fake_A_Ours_HM.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0013_fake_A_CG.png} \\
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0446_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0446_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0446_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0015_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0015_fake_A_Ours_HM.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0015_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0018_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0018_fake_A_Ours.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0018_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0049_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0049_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0049_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0456_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0456_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0456_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0071_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0071_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0071_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0074_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0074_fake_A_Ours.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0074_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0075_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0075_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0075_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0076_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0076_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0076_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0126_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0126_fake_A_Ours_HM.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0126_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0130_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0130_fake_A_Ours_HM.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0130_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0132_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0132_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0132_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0157_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0157_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0157_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0171_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0171_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0171_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0225_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0225_fake_A_Ours.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0225_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0406_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0406_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0406_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0419_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0419_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0419_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0427_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0427_fake_A_Ours_HM.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0427_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0431_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0431_fake_A_Ours.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0431_fake_A_CG.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0432_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0432_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0432_fake_A_CG.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0439_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0439_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0439_fake_A_CG.png} \\

%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0442_real_B.png} & %\includegraphics[width=0.1\linewidth]{Figures/SDOF_0442_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0442_fake_A_CG.png} &

\end{tabular}
\caption{More results of our Depthless unsupervised Bokeh. We depict the input (left most), our result (second column from the left) and Cycle GAN and MUNIT (right column).}
\end{figure*}

\begin{figure*}[ht]
\begin{tabular}{cccccccc}


Input & Ours & CycGAN & MUNIT & Input & Ours & CycGAN & MUNIT\\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0020_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0020_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0020_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0020_fake_A_MUNIT.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0024_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0024_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0024_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0024_fake_A_MUNIT.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0047_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0047_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0047_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0047_fake_A_MUNIT.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0064_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0064_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0064_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0064_fake_A_MUNIT.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0069_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0069_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0069_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0069_fake_A_MUNIT.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0086_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0086_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0086_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0086_fake_A_MUNIT.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0087_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0087_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0087_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0087_fake_A_MUNIT.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0146_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0146_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0146_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0146_fake_A_MUNIT.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0418_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0418_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0418_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0418_fake_A_MUNIT.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0423_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0423_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0423_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0423_fake_A_MUNIT.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0429_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0429_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0429_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0429_fake_A_MUNIT.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0356_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0356_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0356_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0356_fake_A_MUNIT.png} \\

\includegraphics[width=0.1\linewidth]{Figures/SDOF_0453_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0453_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0453_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0453_fake_A_MUNIT.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0458_real_B.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0458_fake_A_Ours.png} &
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0458_fake_A_CG.png} & 
\includegraphics[width=0.1\linewidth]{Figures/SDOF_0458_fake_A_MUNIT.png} \\
\end{tabular}
\caption{Results of our Depthless unsupervised Bokeh. We depict the input (left most), our result (second column from the left) and the competing methods Cycle GAN and MUNIT (two right columns correspondingly).}
\end{figure*}


%\begin{table*}[ht]
%\begin{tabular}{llllllll}
%
%
%Input & Ours & Input & Ours Input & Ours & Input & Ours\\
%
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0007_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0007_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0013_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0013_fake_A_Ours_HM.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0015_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0015_fake_A_Ours_HM.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0018_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0018_fake_A_Ours.png} \\
%
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0049_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0049_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0456_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0456_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0071_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0071_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0074_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0074_fake_A_Ours.png} \\
%
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0075_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0075_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0076_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0076_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0126_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0126_fake_A_Ours_HM.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0130_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0130_fake_A_Ours_HM.png} \\
%
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0132_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0132_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0157_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0157_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0171_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0171_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0225_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0225_fake_A_Ours.png} \\
%
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0406_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0406_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0419_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0419_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0427_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0427_fake_A_Ours_HM.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0431_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0431_fake_A_Ours.png} \\
%
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0432_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0432_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0439_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0439_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0442_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0442_fake_A_Ours.png} &
%\includegraphics[width=0.1\linewidth]{Figures/SDOF_0446_real_B.png} & \includegraphics[width=0.1\linewidth]{Figures/SDOF_0446_fake_A_Ours.png} \\
%
%
%
%\end{tabular}
%\caption{More Results of our Depthless Bokeh}
%\end{table*}


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-sigconf-authordraft.tex \
	samples/sample-sigconf-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-sigconf-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done

samples/sample-manuscript.pdf \
samples/sample-acmsmall.pdf \
samples/sample-acmlarge.pdf \
samples/sample-acmtog.pdf: samples/samplebody-journals.tex

samples/sample-sigconf.pdf \
samples/sample-sigconf-authordraft.pdf \
samples/sample-sigconf-xelatex.pdf \
samples/sample-sigplan.pdf \
samples/sample-sigchi.pdf: samples/samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean
	$(RM) $(PDF) samples/*-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> suppmat.tex <==
\section{Supplementary Material}


\begin{figure*}[ht]
\begin{tabular}{lccc}

& \hspace{5px} Input \hspace{25px} \OurName & \hspace{5px} Input \hspace{25px} \OurName & \hspace{5px} Input \hspace{25px} \OurName \\

\multirow{2}{*}{\vtop{\hbox{\strut Monet $\rightarrow$}\hbox{\strut Photo}}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00010_inputA.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00010_fakeB_IDT3_T3_TIDT6_TCYC6.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00049_inputA.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00049_fakeB_IDT3_T3_TIDT6_TCYC6.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00047_inputA.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00047_fakeB_IDT3_T3_TIDT6_TCYC6.png}} \\

&
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00280_real_A.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00280_fake_B.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00150_real_A.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00150_fake_B.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00430_real_A.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00430_fake_B.png}} \\

\multirow{2}{*}{\vtop{\hbox{\strut Photo $\rightarrow$}\hbox{\strut Monet}}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00040_inputB.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00040_fakeA_IDT3_T3_TIDT6_TCYC6.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00050_inputB.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00050_fakeA_IDT3_T3_TIDT6_TCYC6.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00070_inputB.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00070_fake_A_IDT3_T3_TIDT6_TCYC6.png}} \\

&
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00120_real_B.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00120_fake_A.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00440_real_B.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00440_fake_A.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00450_real_B.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00450_fake_A.png}} \\ \\

\multirow{2}{*}{\vtop{\hbox{\strut Cezanne $\rightarrow$}\hbox{\strut Photo}}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00053_inputA.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00053_fakeB_IDT3_T3_TIDT6_TCYC6.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00084_inputA.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00084_fakeB_IDT3_T3_TIDT6_TCYC6.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00006_inputA.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00006_fakeB_IDT3_T3_TIDT6_TCYC6.png}} \\

&
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00053_real_A.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00053_fake_B.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00087_real_A.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00087_fake_B.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00100_real_A.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00100_fake_B.png}} \\

\multirow{2}{*}{\vtop{\hbox{\strut Photo $\rightarrow$}\hbox{\strut Cezanne}}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00070_inputB.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00070_fake_A_IDT3_T3_TIDT6_TCYC6.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00200_inputB.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00200_fakeA_IDT3_T3_TIDT6_TCYC6.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00510_inputB.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00510_fakeA_IDT3_T3_TIDT6_TCYC6.png}} \\

&
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00510_real_B.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00510_fake_A.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00520_real_B.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00520_fake_A.png}} &
\raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00530_real_B.png}} \raisebox{0\height}{\includegraphics[width=0.125\linewidth]{../Figures/00530_fake_A.png}} \\

\end{tabular}
\caption{A variety of image-to-image translation results of our method (\OurName), applied on style transfer tasks.}
\label{tab:c2VsCG_Supp}
\end{figure*}



\begin{figure*}[ht]
\begin{tabular}{cccc|cccc}

\multicolumn{4}{c}{Specular to Diffuse} & \multicolumn{4}{c}{Diffuse to Specular} \\

Input & \OurName & Input & \OurName & Input & \OurName & Input & \OurName \\

\includegraphics[width=0.1\linewidth]{../Figures/angel34_512_1035_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/angel34_512_1035_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0408_4_5__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0408_4_5__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0970_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0970_4_5__512_fake_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0345_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0345_4_5__512_fake_A.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/IMG_0564_4_5__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0564_4_5__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0316__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0316__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0408_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0408_4_5__512_fake_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0220_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0220_4_5__512_fake_A.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/IMG_0533_4_5__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0533_4_5__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0415__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0415__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_1308__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_1308__512_fake_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0377_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0377_4_5__512_fake_A.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/angel34_512_1035_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/angel34_512_1035_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/angel34_512_1063_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/angel34_512_1063_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0220_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0220_4_5__512_fake_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0252_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0252_4_5__512_fake_A.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/IMG_0002_4_5__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0002_4_5__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0408_4_5__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0408_4_5__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0283_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0283_4_5__512_fake_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0314_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0314_4_5__512_fake_A.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0275__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0275__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0627_4_5__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0627_4_5__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0345_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0345_4_5__512_fake_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0377_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0377_4_5__512_fake_A.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/IMG_0533_4_5__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0533_4_5__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0415__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0415__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0408_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0408_4_5__512_fake_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0003__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0003__512_fake_A.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/IMG_0564_4_5__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0564_4_5__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0316__512_real_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_0316__512_fake_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0970_4_5__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/IMG_0970_4_5__512_fake_A.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_1308__512_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/jeIMG_1308__512_fake_A.png} \\

\end{tabular}
\caption{Results of our Specular to Diffuse: The odd colums show the inputs while the even ones show our output. The four left most columns depict a translation form a specular input to a diffuse output, while the four right rows show the opposite direction of translation.}
\end{figure*}

%\includegraphics[width=0.3\linewidth]{../Figures/ElephantWOBG_0110_real_B.png} &
%\includegraphics[width=0.3\linewidth]{../Figures/ElephantWOBG_0110_fake_A_procd.png} &
%\includegraphics[width=0.3\linewidth]{../Figures/ElephantWOBG_0110_fake_A_procd_CG.png} \\

%\includegraphics[width=0.3\linewidth]{../Figures/ElephantWOBG_0122_real_B.png} &
%\includegraphics[width=0.3\linewidth]{../Figures/ElephantWOBG_0122_fake_A_procd.png} &
%\includegraphics[width=0.3\linewidth]{../Figures/ElephantWOBG_0122_fake_A_procd_CG.png} \\

\begin{figure*}[ht]
\begin{tabular}{ccccc}

Input & \OurName & CycleGAN & MUNIT & DPED \\

\includegraphics[width=0.175\linewidth]{../Figures/107_real_A_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/107_fake_B_Ours_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/107_fake_B_CG_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/107_fake_B_MUNIT_Overlay.png} & 
\includegraphics[width=0.175\linewidth]{../Figures/107_fake_B_DPED_Overlay.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/107_real_A_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/107_fake_B_Ours_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/107_fake_B_CG_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/107_fake_B_MUNIT_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/107_fake_B_DPED_Zoom.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/1002_real_A_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1002_fake_B_Ours_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1002_fake_B_CG_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1002_fake_B_MUNIT_Overlay.png} & 
\includegraphics[width=0.175\linewidth]{../Figures/1002_fake_B_DPED_Overlay.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/1002_real_A_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1002_fake_B_Ours_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1002_fake_B_CG_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1002_fake_B_MUNIT_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1002_fake_B_DPED_Zoom.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/1042_real_A_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1042_fake_B_Ours_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1042_fake_B_CG_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1042_fake_B_MUNIT_Overlay.png} & 
\includegraphics[width=0.175\linewidth]{../Figures/1042_fake_B_DPED_Overlay.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/1042_real_A_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1042_fake_B_Ours_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1042_fake_B_CG_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1042_fake_B_MUNIT_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1042_fake_B_DPED_Zoom.png} \\


\end{tabular}
\caption{Results of employing \OurName for enhancing a mobile phone photo to DSLR quality. We show the input, our result, Cycle GAN's, MUNIT's and DPED's results, from left to right. The odd rows show the full images, while the even rows show a zoom-in.}
\end{figure*}


\begin{figure*}[ht]
\begin{tabular}{ccccc}

Input & \OurName & CycleGAN & MUNIT & DPED \\

\includegraphics[width=0.175\linewidth]{../Figures/1046_real_A_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1046_fake_B_Ours_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1046_fake_B_CG_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1046_fake_B_MUNIT_Overlay.png} & 
\includegraphics[width=0.175\linewidth]{../Figures/1046_fake_B_DPED_Overlay.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/1046_real_A_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1046_fake_B_Ours_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1046_fake_B_CG_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1046_fake_B_MUNIT_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1046_fake_B_DPED_Zoom.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/1068_real_A_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1068_fake_B_Ours_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1068_fake_B_CG_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1068_fake_B_MUNIT_Overlay.png} & 
\includegraphics[width=0.175\linewidth]{../Figures/1068_fake_B_DPED_Overlay.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/1068_real_A_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1068_fake_B_Ours_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1068_fake_B_CG_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1068_fake_B_MUNIT_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1068_fake_B_DPED_Zoom.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/1071_real_A_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1071_fake_B_Ours_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1071_fake_B_CG_Overlay.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1071_fake_B_MUNIT_Overlay.png} & 
\includegraphics[width=0.175\linewidth]{../Figures/1071_fake_B_DPED_Overlay.png} \\

\includegraphics[width=0.175\linewidth]{../Figures/1071_real_A_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1071_fake_B_Ours_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1071_fake_B_CG_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1071_fake_B_MUNIT_Zoom.png} &
\includegraphics[width=0.175\linewidth]{../Figures/1071_fake_B_DPED_Zoom.png} \\

\end{tabular}
\caption{Results of employing \OurName for enhancing a mobile phone photo to DSLR quality. We show the input, our result, Cycle GAN's, MUNIT's and DPED's results, from left to right. The odd rows show the full images, while the even rows show a zoom-in.}
\end{figure*}



\begin{figure*}[ht]
\begin{tabular}{cccc|cccc}

Input & \OurName & CycleGAN & GrabCut & Input & \OurName & CycleGAN & GrabCut \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0004_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0004_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0004_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0004_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0018_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0018_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0018_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0018_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0054_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0054_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0054_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0054_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0056_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0056_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0056_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0056_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0062_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0062_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0062_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0062_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0063_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0063_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0063_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0063_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0067_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0067_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0067_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0067_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0083_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0083_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0083_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0083_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0121_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0121_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0121_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0121_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0138_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0138_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0138_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0138_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0211_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0211_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0211_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0211_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0150_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0150_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0150_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0150_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0153_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0153_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0153_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0153_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0155_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0155_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0155_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0155_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0157_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0157_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0157_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0157_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0160_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0160_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0160_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0160_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0161_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0161_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0161_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0161_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0168_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0168_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0168_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0168_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0189_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0189_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0189_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0189_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0181_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0181_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0181_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0181_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0198_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0198_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0198_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0198_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0208_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0208_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0208_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0208_fake_A_Grabcut.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0218_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0218_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0218_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0218_fake_A_Grabcut.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0230_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0230_fake_A_procd.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0230_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/ElephantWOBG_0230_fake_A_Grabcut.png} \\

\end{tabular}
\caption{Results of employing \OurName for foreground extraction applied on elephant photos. From left to right, we show the input image, CrossNet, CycleGAN and GrabCut.}
\end{figure*}



\begin{figure*}[ht]
\begin{tabular}{cccc|cccc}

Input & \OurName & CycleGAN & AGGAN & Input & \OurName & CycleGAN & AGGAN \\

\includegraphics[width=0.1\linewidth]{../Figures/102121_287_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/102121_287_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/102121_287_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/102121_287_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/104676_189953_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/104676_189953_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/104676_189953_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/104676_189953_fake_A_procd_AGGAN.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/104676_617_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/104676_617_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/104676_617_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/104676_617_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/104676_9_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/104676_9_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/104676_9_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/104676_9_fake_A_procd_AGGAN.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/7538282_225096_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7538282_225096_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7538282_225096_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7538282_225096_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/7212450_20_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_20_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_20_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_20_fake_A_procd_AGGAN.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/7212450_364920_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_364920_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_364920_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_364920_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/7212459_691_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212459_691_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212459_691_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212459_691_fake_A_procd_AGGAN.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/7271610_11_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7271610_11_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7271610_11_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7271610_11_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/7373491_4697_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7373491_4697_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7373491_4697_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7373491_4697_fake_A_procd_AGGAN.png} \\


\includegraphics[width=0.1\linewidth]{../Figures/7161124_20_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7161124_20_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7161124_20_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7161124_20_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/7212450_303655_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_303655_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_303655_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_303655_fake_A_procd_AGGAN.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/7571295_10623_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7571295_10623_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7571295_10623_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7571295_10623_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/7212450_366115_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_366115_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_366115_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7212450_366115_fake_A_procd_AGGAN.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/7567515_9_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7567515_9_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7567515_9_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7567515_9_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/7425142_3575_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7425142_3575_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7425142_3575_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7425142_3575_fake_A_procd_AGGAN.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/7158233_3_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7158233_3_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7158233_3_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7158233_3_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/7159690_89459_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7159690_89459_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7159690_89459_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7159690_89459_fake_A_procd_AGGAN.png} \\

\includegraphics[width=0.1\linewidth]{../Figures/7297622_352714_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7297622_352714_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7297622_352714_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7297622_352714_fake_A_procd_AGGAN.png} &

\includegraphics[width=0.1\linewidth]{../Figures/7289535_4697_real_B.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7289535_4697_fake_A_procd_Ours.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7289535_4697_fake_A_procd_CG.png} &
\includegraphics[width=0.1\linewidth]{../Figures/7289535_4697_fake_A_procd_AGGAN.png} \\


\end{tabular}
\caption{Results of employing \OurName for foreground extraction applied on the UT Zappos50K dataset. From left to right, we show the input image, CrossNet, CycleGAN and AGGAN.}
\end{figure*}


\begin{figure*}[ht]
\begin{tabular}{ccc|ccc}

Input & Ground Truth & \OurName & Input & Ground Truth & \OurName \\

\includegraphics[width=0.13\linewidth]{../Figures/2007_003022_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_003022_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_003022_fake_A_procd.png} &

\includegraphics[width=0.13\linewidth]{../Figures/2007_005114_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_005114_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_005114_fake_A_procd.png} \\

\includegraphics[width=0.13\linewidth]{../Figures/2007_006364_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_006364_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_006364_fake_A_procd.png} &

\includegraphics[width=0.13\linewidth]{../Figures/2008_002459_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2008_002459_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2008_002459_fake_A_procd.png} \\

\includegraphics[width=0.13\linewidth]{../Figures/2007_008142_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_008142_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_008142_fake_A_procd.png} &

\includegraphics[width=0.13\linewidth]{../Figures/2007_008256_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_008256_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_008256_fake_A_procd.png} \\

\includegraphics[width=0.13\linewidth]{../Figures/2007_008307_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_008307_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_008307_fake_A_procd.png} &

\includegraphics[width=0.13\linewidth]{../Figures/2007_008802_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_008802_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_008802_fake_A_procd.png} \\

\includegraphics[width=0.13\linewidth]{../Figures/2007_009251_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_009251_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_009251_fake_A_procd.png} &

\includegraphics[width=0.13\linewidth]{../Figures/2007_009807_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_009807_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_009807_fake_A_procd.png} \\

\includegraphics[width=0.13\linewidth]{../Figures/2008_000141_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2008_000141_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2008_000141_fake_A_procd.png} &

\includegraphics[width=0.13\linewidth]{../Figures/2008_000219_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2008_000219_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2008_000219_fake_A_procd.png} \\

\includegraphics[width=0.13\linewidth]{../Figures/2008_005928_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2008_005928_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2008_005928_fake_A_procd.png} &

\includegraphics[width=0.13\linewidth]{../Figures/2007_002273_real_B.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_002273_real_A.png} &
\includegraphics[width=0.13\linewidth]{../Figures/2007_002273_fake_A_procd.png} \\

\end{tabular}
\caption{Results of employing \OurName for foreground extraction applied on horse photos from the HDSeg dataset. From left to right, we show the input image, the ground truth and \OurName's results.}
\end{figure*}





